Higher-order Sparse Convolutions in Graph Neural Networks

Graph Neural Networks (GNNs) have been applied to many problems in computer sciences. Capturing higher-order relationships between nodes is crucial to increase the expressive power of GNNs. However, existing methods to capture these relationships could be infeasible for large-scale graphs. In this work, we introduce a new higher-order sparse convolution based on the Sobolev norm of graph signals. Our Sparse Sobolev GNN (S-SobGNN) computes a cascade of filters on each layer with increasing Hadamard powers to get a more diverse set of functions, and then a linear combination layer weights the embeddings of each filter. We evaluate S-SobGNN in several applications of semi-supervised learning. S-SobGNN shows competitive performance in all applications as compared to several state-of-the-art methods.

==> old_stuff.tex <==
\begin{table}[]
\centering
\caption{Accuracy (in \%) for several previous methods and our S-SobGNN algorithm in four datasets for semi-supervised learning, inferring the graphs with a $k$-NN method.}
\label{tbl:results_classification}
\begin{threeparttable}
\makebox[\linewidth]{
\scalebox{0.708}{
\begin{tabular}{r|cccc}
\toprule
\textbf{Model} & \textbf{Cancer} & \textbf{20News} & \textbf{HAR} & \textbf{Isolet} \\
\midrule
Cheby \cite{defferrard2016convolutional} & \color{blue} $\textbf{84.37} \pm \textbf{3.82}$ & $53.08 \pm 1.44$ & $34.84 \pm 2.88$ & $9.26 \pm 1.18$ \\
GCN \cite{kipf2017semi} & $74.51 \pm 4.99$ & $45.59 \pm 3.00$ & \color{blue} $\textbf{65.39} \pm \textbf{5.72}$ & \color{blue} $\textbf{52.85} \pm \textbf{2.75}$ \\
GAT \cite{velickovic2018graph} & $71.26 \pm 5.18$ & $46.31 \pm 2.39$ & $47.81 \pm 5.39$ & $45.69 \pm 4.01$ \\
SGC \cite{wu2019simplifying} & $68.83 \pm 4.69$ & $45.87 \pm 2.57$ & $33.94 \pm 2.13$ & $21.69 \pm 1.69$ \\
k-GNN \cite{morris2019weisfeiler} & $60.18 \pm 4.00$ & $18.71 \pm 2.93$ & $21.59 \pm 1.82$ & $8.13 \pm 0.96$ \\
ClusterGCN \cite{chiang2019cluster} & $79.17 \pm 4.47$ & \color{blue} $\textbf{59.03 }\pm \textbf{2.05}$ & $45.97 \pm 4.36$ & $16.52 \pm 2.81$ \\
Transformer \cite{shi2021masked} & $71.32 \pm 4.80$ & $48.92 \pm 0.25$ & $47.80 \pm 4.53$ & $25.97 \pm 3.14$ \\
\midrule
S-SobGNN (ours) & \color{red} $\textbf{92.58} \pm \textbf{0.43}$ & \color{red} $\textbf{69.68} \pm \textbf{0.44}$ & \color{red} $\textbf{82.81} \pm \textbf{4.43}$ & \color{red} $\textbf{60.69} \pm \textbf{5.57}$ \\
\bottomrule
\end{tabular}
}
}
\begin{tablenotes}\footnotesize
\item \scriptsize \hspace{0.15cm} The best and second-best performing methods on each dataset are shown in {\color{red}\textbf{red}}\\and {\color{blue}\textbf{blue}}, respectively.
\end{tablenotes}
\end{threeparttable}
\end{table}
